Why do LLaVA Vision-Language Models Reply to Images in English?

We uncover a surprising multilingual bias occurring in a popular class of multimodal vision-language models (VLMs). Including an image in the query to a LLaVA-style VLM significantly increases the likelihood of the model returning an English response, regardless of the language of the query. This paper investigates the causes of this loss with a two-pronged approach that combines extensive ablation of the design space with a mechanistic analysis of the models' internal representations of image and text inputs. Both approaches indicate that the issue stems in the language modelling component of the LLaVA model. Statistically, we find that switching the language backbone for a bilingual language model has the strongest effect on reducing this error. Mechanistically, we provide compelling evidence that visual inputs are not mapped to a similar space as text ones, and that intervening on intermediary attention layers can reduce this bias. Our findings provide important insights to researchers and engineers seeking to understand the crossover between multimodal and multilingual spaces, and contribute to the goal of developing capable and inclusive VLMs for non-English contexts.

==> documentBody/09-tech_explainers.tex <==
%%%%%
% MH: Moved this to SI.tex
%%%%%
%\subsection{Primer on LLaVA}
%\paragraph{What is LLaVA?}
%
%Our study analyzes LLaVA, a multimodal model (VLM) that integrates a pretrained vision encoder, denoted as $E_V$, with a large language model (LLM), using a connecting multilayer perceptron (MLP). The process is defined in two main training stages: pretraining of the MLP and joint finetuning of the MLP with the LLM.
%
%\paragraph{Model Architecture}
%The VLM comprises the following components:
%
%\textit{Vision Encoder:} The vision encoder $E_V$ processes the visual input $X_v$ to produce a set of embeddings $E_V(X_v)$.
%
%\textit{MLP Connector:} A connecting MLP, defined as $F$, transforms the output of $E_V$ into the dimenstionality of the LLM. This transformation is represented as $F(E_V(X_v))$.
%
%\textit{LLM:} The LLM processes both textual query $X_q$ and the transformed vision embeddings. The combined input to the LLM is given by concatenating the embeddings from the MLP with text embeddings, i.e., $LLM([F(E_V(X_v)); E_L(X_q)])$, where $E_L$ denotes 
%
%The VLM is defined as a function that takes an image input $X_v$ and a textual question $X_q$, and processes these through the vision encoder, MLP connector $F$, and LLM to produce an output $X_a$, which is the model's answer to the question based on the visual context. Formally, the VLM can be expressed as:
%\begin{equation}
%    VLM(X_v, X_q) = LLM\left([\text{F}(E_V(X_v)); E_L(X_q)]\right),
%\end{equation}
%where $E_V(X_v)$ is the output of the vision encoder for the input image, $\text{F}(E_V(X_v))$ is the transformed visual embedding suitable for the LLM, and $E_L(X_q)$ represents the embedded form of the textual question. The final output $X_a$ is generated by the LLM, which synthesizes and integrates both the visual and textual information to produce a contextually appropriate answer.
%
%\paragraph{Training Procedure}
%The training of the VLM is structured into two distinct stages: pretraining and finetuning.
%During the pretraining stage, the MLP is trained while keeping $E_V$ and the LLM frozen. The objective is to optimize the MLP to map the vision encoder outputs to a representation that is effectively integrable with the LLM. The training uses a custom dataset of 595k samples filtered from CC3M \cite{sharma-etal-2018-conceptual}:
%\begin{equation}
%    \mathcal{L}_{\text{MLP}} = \sum_{(X_v, X_c) \in \mathcal{D}} L_{CE}(VLM(X_v, X_q)),
%\end{equation}
%where $X_c$ represents the captions associated with $X_v$, and $\mathcal{D}$ denotes the dataset.
%
%\paragraph{Finetuning}
%In the finetuning stage, the MLP and the LLM are jointly trained with a larger, diverse dataset of 665k multimodal instruction tuning examples, integrating both synthetic and established vision-language training sets. The entire conversation $C = (X_q, X_a)$ is fed into the LLM, with autoregressive masking applied to focus training on the answers using supervised cross-entropy loss $L_{CE}$:
%\begin{equation}
%    \mathcal{L}_{\text{VLM}} = \sum_{C \in \mathcal{C}} L_{CE}(VLM(X_v, X_q)),
%\end{equation}
%where $\mathcal{C}$ represents the conversation dataset, and training focuses exclusively on the answer parts $X_a$, leveraging the context provided by the entire conversation but training only through the answer segments.
%

==> documentBody/10-datasets.tex <==

Here we provide an overview on the datasets we employ in our study.
\label{sec:related_work_ml_mm_datasets}
%
%\begin{table}[ht!]
%\centering
%\caption{Overview of the employed datasets.}
%\label{tab:dataset_summary}
%    \begin{tabular}{llrr}
%        \toprule
%        \textbf{Dataset} & \textbf{MM} & \multicolumn{1}{l}{\textbf{\#Langs.}} & \multicolumn{1}{l}{\textbf{Size}}  \\
%        \midrule
%        MaXM     & yes & $7$ & $2142$     \\
%        ViSIT     & yes & $10$ & $5740$     \\
%        PALO-LLaVAW    & yes & $10$ & $6000$     \\
%        MultiQ    & text-only & $137$ & $27400$    \\
%        \bottomrule
%    \end{tabular}
%\end{table}
%
\paragraph{MaXM} was introduced by~\citet{changpinyo2023maxm} and is a VQA dataset comprising seven languages in five scripts.
%
In MaXM, the questions and their respective answers are in the same language.
%
Moreover, in MaXM, the images are a subset of the XM3600~\citep{thapliyal2022xm3600} dataset and are chosen to match a region where the language of the question-answer pair is spoken.
%
To increase the cultural diversity, the images selected to match the region where the language of the question-answer pair is spoken.
%


\paragraph{VisIT-Bench} stands for \textbf{Vis}ual \textbf{I}nstruction \textbf{T}uning \textbf{Bench}mark~\cite{bitton2023visit}.
%
The dataset consists of $592$ vision-language tasks written by human researchers, with GPT-4-generated responses and dense instruction-conditioned captions of the image that are rated by human coders.
%
The $562$ images are taken from the OpenImages~\cite{kuznetsova2020openimages} v7 dataset.
%
In this work we use $525$ examples where the GPT-4 generated responses are rated as correct by human annotators.
%
We machine translate these examples into Arabic, Bengali, Chinese, German, Hebrew, Hindi, Japanese, Spanish and Thai using the Azure Translation API.

%In this work, we used the $574$ samples, where the GPT-4 is considered correct and translated the instructions and responses into $10$ languages using the Bing translate API.
%

\paragraph{PALO-LLaVA-Bench-In-The-Wild} dataset is a multilingual VQA dataset created by the PALO authors ~\cite{maaz2024palo} by machine translating the original LLaVA-Bench-In-The-Wild~\cite{liu2023llava} in $10$ languages using a fine-tuned GPT-3.5 instance.
%
The dataset comprises of $60$ questions per language considering $24$ diverse images with a caption describing the visual content.
%
\paragraph{MultiQ} is an evaluation dataset for open-ended question answering covering 137 typologically diverse languages. It is specifically constructed to only contain questions that are simple, factual, and target common knowledge to only test the multilingual capabilities of language models, and no complex reasoning \cite{holtermann2024evaluating}.



==> documentBody/11-models.tex <==
Here we provide an overview of the models we employed in our study.

\paragraph{OpenAI/CLIP} is a jointly optimized vision and text feature extractor  trained using large-scale image-caption pairs \cite{radford_learning_2021}. 
CLIP is focused on learning image representations from scratch that are trivially transferable to many downstream tasks without the need for domain specific training. 

\paragraph{DINOv2} is a series of image encoders trained on curated data using unsupervised learning \cite{oquab2024dinov2}. 
Through an improved training recipe and larger dataset, followed by a distillation process of larger to smaller models, DINOv2 is positioned as a ViT-based general-purpose image encoder that surpasses OpenAI/CLIP on most benchmarks.

\paragraph{LLaVA-v1.5} is a large multimodal model trained end-to-end with visual instruction following \cite{liu2023llava}.
The model combines a vision model --- OpenAI/CLIP --- with a large language model --- Vicuna-v1.5 --- achieving impressive visual and language understanding results that were state-of-the-art at its release. 
In this work we used the 7b and 13b variants of the model.

\paragraph{BakLLaVA} is a large multimodal model based on the LLaVA-v1.5 architecture using Mistral-7b as the base LLM \cite{skunkworksai2023bakllava1}.
The model utilizes training data from LLaVA-v1.5 as well as additional sources including ShareGPT and private data with a permissive license.

\paragraph{Yi-6b-chat} is a large language model trained from scratch on English and Chinese corpora \cite{ai2024yi}. 
In this work, we use the 6b variant that has been extended with chat-style training. 

\paragraph{Leo-7b-chat} is a large language model that extends Llama-2 into German through continued training on a large German corpus \cite{pluster2023leolm}. 

\paragraph{GlotLID v3} is a language identification model that coveres 2102 languages. 
The data used to train this model was sourced from Wikipedia, news sites,
translation corpora, religious text, and storybooks. 

\paragraph{NLLB-1.7-distilled} is translation model that support direct translation between 200 languages, including many low-resource languages \cite{nllbteam2022language}. 
The datasets used to train NLLB (No Language Left Behind) were sourced from professionally translated sentences in the Wikipedia domain in addition to publicly available translation datasets. 


==> documentBody/12-tables-figures.tex <==

\paragraph{Prevalence}


\begin{table}[]
    \centering
    \small
    \addtolength{\tabcolsep}{-0.3em}
    \begin{tabular}{l|l|c|c|c|c}
    \toprule
     \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Lang.}}  & \multicolumn{4}{c}{\textbf{Evaluation Dataset} } \\  
  &  & llavaw & maxm & visitazure & multiq  \\  
  \midrule
&ar  &  -0.02 &   --  &  0.01  & 0.40  \\
&bn  &  0.07  & -- &  0.02  &  0.35  \\
&zh  &  0.05 & 0.17  &  0.04  &  0.27  \\
&fr  &  0.13  & 0.33  & -- & 0.16  \\
&de  & -- & -- &  0.13  & 0.23  \\
&he  & -- & 0.00  &  0.00 &  0.22  \\
baklava & hi  &  0.00 & -0.01  &  0.02 &  0.30  \\
&ja  &  0.00 & -- &  0.04 &  0.21  \\
&ro  & -- & 0.57  & -- &  0.08  \\
&ru  &  0.00 & -- &  --  &  0.29  \\
&es  &  0.13 & -- & 0.16 &  0.26  \\
&th  & -- & 0.14 & 0.01 &  0.43  \\
&ur  &  0.00 & -- & -- &  0.48  \\
\midrule
&ar  &  0.23 & -- &  0.02 &  0.01  \\
  &bn  &  0.12 & -- & 0.09  & 0.01  \\
  &zh  &  0.23 & 0.00 & 0.02  & 0.00  \\
  &fr  &  0.17 & -0.00  & -- &  0.01  \\
  &de  & -- & -- & 0.05 &  0.00  \\
  &he  & -- & 0.13  & 0.04  & 0.01  \\
llava7b  &hi  &  0.13 & 0.04  & 0.03  & 0.00  \\
  &ja  &  0.12 & -- & 0.02  & 0.00  \\
  &ro  & -- & 0.02  & -- &  0.00  \\
  &ru  &  0.23 & -- & -- & -0.01  \\
  &es  &  0.20 & -- &  0.02  & 0.00  \\
  &th& --  & 0.00  &  0.05  & 0.00  \\
  &ur  &  -0.03 & -- & -- & 0.01  \\
  \midrule
  &  ar  &  0.18   & -- &  0.17 &  0.01  \\
&  bn  &  0.25 & -- &  0.24  & 0.03  \\
&  zh  &  0.15 & 0.04  &  0.07 &  0.01  \\
&  fr  &  0.20 & 0.01  & -- & 0.01  \\
&  de  & -- & -- &  0.10  & 0.02  \\
&  he  & -- & 0.17  &  0.13  & 0.01  \\
llava13b &  hi  &  0.32 & 0.05  &  0.13  & 0.02  \\
&  ja  &  0.18 & -- &  0.05  & 0.02  \\
&  ro  & -- & 0.11 & -- & 0.13  \\
&  ru  &  0.45 & -- & -- & 0.08  \\
&  es  &  0.22  & -- &  0.05 &  0.00  \\
&  th  & -- & 0.15  &  0.26  & 0.07  \\
&  ur  &  0.58 & -- & -- &  0.03  \\
\midrule
  &  ar  &  0.58 & -- &  0.54 & 0.21  \\
&  bn  &  0.43 & -- &  0.42  & 0.17  \\
&  zh  &  0.68 & 0.68  &  0.64 &  0.25  \\
&  fr  &  0.77 & 0.62  & -- &  0.21  \\
&  de  & -- & -- &  0.64  & 0.28  \\
&  he  & -- & 0.58  &  0.58 &  0.15  \\
llava- &  hi  &  0.43 & 0.56  &  0.54  & 0.32  \\
gemma2b&  ja  &  0.53 & -- &  0.47  & 0.32  \\
&  ro  & -- & 0.36  & --  &  0.08  \\
&  ru  &  0.88 & -- & --  &  0.54  \\
&  es  &  0.78 & -- &  0.75  & 0.42  \\
&  th  & -- & 0.53  & 0.44  & 0.21  \\
&  ur  &  0.47 & -- & -- & 0.21  \\
\bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:raw_fidelity}
\end{table}



\begin{table}[]
\begin{tabular}{lllll}
llava7b    &          &        &              &            \\
dataset    &   Lang.  & IFL    & \begin{tabular}[c]{@{}c@{}}IFL + \\ Remedy\end{tabular} & Diff. \\ \hline
llavaw     & ar     & -0.250 & -0.083       & 0.167      \\
           & bn     & -0.117 & -0.050       & 0.067      \\
           & zh     & -0.233 & -0.017       & 0.217      \\
           & fr     & -0.183 & 0.000        & 0.183      \\
           & hi     & -0.133 & -0.033       & 0.100      \\
           & ja     & -0.117 & -0.050       & 0.067      \\
           & ru     & -0.233 & -0.017       & 0.217      \\
           & es     & -0.200 & -0.050       & 0.150      \\
           & ur     & -0.050 & 0.083        & 0.133      \\ \hline
maxm       & zh     & 0.004  & 0.000        & -0.004     \\
           & fr     & 0.004  & -0.011       & -0.015     \\
           & he     & -0.132 & -0.125       & 0.007      \\
           & hi     & -0.042 & -0.035       & 0.008      \\
           & ro     & 0.000  & -0.014       & -0.014     \\
           & th     & -0.007 & -0.011       & -0.004     \\ \hline
visitazure & ar     & -0.038 & -0.047       & -0.009     \\
           & bn     & -0.084 & -0.038       & 0.045      \\
           & zh     & -0.026 & -0.047       & -0.021     \\
           & de     & -0.054 & -0.037       & 0.017      \\
           & he     & -0.038 & -0.037       & 0.002      \\
           & hi     & -0.026 & -0.009       & 0.017      \\
           & ja     & -0.021 & -0.051       & -0.030     \\
           & es     & -0.024 & -0.042       & -0.017     \\
           & th     & -0.045 & -0.010       & 0.035      \\ \hline
average    &  -     & -0.085 & -0.030       & 0.055     \\ \hline
\end{tabular}
\caption{mechint raw llava7b scores. }
    \label{tab:mechint_raw_llava7b}
\end{table}

\begin{table}[]
\begin{tabular}{ccccc}
llava13b   &          &        &              &            \\
dataset    &   Lang.  & IFL    & \begin{tabular}[c]{@{}c@{}}IFL + \\ Remedy\end{tabular} & Diff. \\ \hline
llavaw     & ar     & -0.183 & -0.033       & 0.150      \\
           & bn     & -0.233 & -0.083       & 0.150      \\
           & zh     & -0.133 & -0.033       & 0.100      \\
           & fr     & -0.200 & -0.100       & 0.100      \\
           & hi     & -0.317 & -0.200       & 0.117      \\
           & ja     & -0.183 & -0.117       & 0.067      \\
           & ru     & -0.433 & -0.317       & 0.117      \\
           & es     & -0.233 & -0.183       & 0.050      \\
           & ur     & -0.550 & -0.267       & 0.283      \\ \hline
maxm       & zh     & -0.025 & -0.007       & 0.018      \\
           & fr     & -0.008 & -0.045       & -0.038     \\
           & he     & -0.175 & -0.121       & 0.054      \\
           & hi     & -0.042 & -0.035       & 0.008      \\
           & ro     & -0.106 & -0.085       & 0.021      \\
           & th     & -0.157 & -0.093       & 0.063      \\ \hline
visitazure & ar     & -0.174 & -0.066       & 0.108      \\
           & bn     & -0.244 & -0.136       & 0.108      \\
           & zh     & -0.071 & -0.031       & 0.040      \\
           & de     & -0.105 & -0.094       & 0.010      \\
           & he     & -0.125 & -0.082       & 0.044      \\
           & hi     & -0.136 & -0.096       & 0.040      \\
           & ja     & -0.056 & -0.044       & 0.012      \\
           & es     & -0.057 & -0.042       & 0.016      \\
           & th     & -0.258 & -0.155       & 0.103      \\ \hline
average    &  -     & -0.175 & -0.103       & 0.073      \\ \hline
\end{tabular}
\caption{mechint raw llava13b scores. }
    \label{tab:mechint_raw_llava13b}
\end{table}

\begin{table}[]
\begin{tabular}{ccccc}
bakllava   &          &        &              &            \\
dataset    &   Lang.  & IFL    & \begin{tabular}[c]{@{}c@{}}IFL + \\ Remedy\end{tabular} & Diff. \\ \hline
llavaw     & ar     & 0.000  & 0.350        & 0.350      \\
           & bn     & -0.050 & 0.217        & 0.267      \\
           & zh     & -0.033 & -0.067       & -0.033     \\
           & fr     & -0.117 & 0.000        & 0.117      \\
           & hi     & 0.000  & 0.050        & 0.050      \\
           & ja     & -0.017 & -0.067       & -0.050     \\
           & ru     & 0.000  & 0.000        & 0.000      \\
           & es     & -0.117 & 0.217        & 0.333      \\
           & ur     & -0.017 & 0.183        & 0.200      \\ \hline
maxm       & zh     & -0.018 & 0.014        & 0.032      \\
           & fr     & -0.318 & -0.223       & 0.095      \\
           & he     & 0.000  & 0.029        & 0.029      \\
           & hi     & 0.000  & 0.135        & 0.135      \\
           & ro     & -0.567 & -0.299       & 0.268      \\
           & th     & -0.119 & -0.078       & 0.041      \\ \hline
visitazure & ar     & -0.010 & 0.608        & 0.618      \\
           & bn     & -0.012 & 0.557        & 0.570      \\
           & zh     & -0.007 & 0.019        & 0.026      \\
           & de     & -0.136 & -0.108       & 0.028      \\
           & he     & 0.000  & 0.078        & 0.078      \\
           & hi     & -0.007 & 0.113        & 0.120      \\
           & ja     & -0.014 & 0.026        & 0.040      \\
           & es     & -0.183 & 0.291        & 0.474      \\
           & th     & -0.007 & 0.294        & 0.301      \\ \hline
average    &  -     & -0.073 & 0.098        & 0.170      \\ \hline
\end{tabular}
\caption{mechint raw bakllava scores. }
    \label{tab:mechint_raw_bakllava}
\end{table}

\begin{table}[]
\begin{tabular}{ccccc}
\multicolumn{2}{c}{llavagemma2b} &        &              &            \\
dataset    &   Lang.  & IFL    & \begin{tabular}[c]{@{}c@{}}IFL + \\ Remedy\end{tabular} & Diff. \\ \hline
llavaw           & ar     & -0.583 & -0.533       & 0.050      \\
                 & bn     & -0.483 & -0.483       & 0.000      \\
                 & zh     & -0.733 & -0.567       & 0.167      \\
                 & fr     & -0.800 & -0.433       & 0.367      \\
                 & hi     & -0.500 & -0.317       & 0.183      \\
                 & ja     & -0.600 & -0.650       & -0.050     \\
                 & ru     & -0.883 & -0.650       & 0.233      \\
                 & es     & -0.900 & -0.700       & 0.200      \\
                 & ur     & -0.517 & -0.483       & 0.033      \\ \hline
maxm             & zh     & -0.852 & -0.762       & 0.090      \\
                 & fr     & -0.905 & -0.652       & 0.254      \\
                 & he     & -0.768 & -0.482       & 0.286      \\
                 & hi     & -0.731 & -0.546       & 0.185      \\
                 & ro     & -0.810 & -0.637       & 0.173      \\
                 & th     & -0.646 & -0.455       & 0.190      \\ \hline
visitazure       & ar     & -0.718 & -0.578       & 0.139      \\
                 & bn     & -0.483 & -0.420       & 0.063      \\
                 & zh     & -0.672 & -0.552       & 0.120      \\
                 & de     & -0.688 & -0.258       & 0.430      \\
                 & he     & -0.617 & -0.280       & 0.336      \\
                 & hi     & -0.589 & -0.375       & 0.214      \\
                 & ja     & -0.526 & -0.509       & 0.017      \\
                 & es     & -0.793 & -0.608       & 0.185      \\
                 & th     & -0.538 & -0.373       & 0.166      \\ \hline
 average         &  -     & -0.681 & -0.513       & 0.168      \\ \hline
\end{tabular}
\caption{mechint raw llava gemma 2b scores. }
    \label{tab:mechint_raw_llava_gemma}
\end{table}
